White Dwarfs with Infrared Excess from DESI EDR

Infrared (IR) excess emission around white dwarfs (WDs) is commonly attributed to circumstellar debris disks and/or low-mass companions, providing a unique window into the evolution of planetary systems and binary evolution after the main-sequence stage. Based on a spectroscopically confirmed WD sample from the DESI Early Data Release, we performed a systematic search for IR excess by combining multi-band photometry from SDSS, Pan-STARRS, UKIDSS, 2MASS, and WISE. Using spectral energy distribution (SED) fitting, we initially identified 72 IR-excess candidates and conducted a stringent contamination assessment based on higher-resolution imaging within 6 arcseconds of each target. After removing sources affected by blending or source confusion, we obtained a final sample of 62 reliable IR excess candidates. Among them, we identify three candidate WD+M dwarf binaries (two new systems), five candidate WD+brown dwarf (BD) binaries (all new), 38 candidate WD+dust disks (28 new), and 16 ambiguous systems that could be either WD+BD or WD+dust (15 new). Compared with previous samples, our catalog extends the parameter space of known dusty WDs toward older cooling ages. Due to the limited spatial resolution of WISE, follow-up high-resolution imaging and/or infrared spectroscopy is required to confirm the physical nature of all candidate systems and to further expand the parameter space of dust disks in terms of cooling age and other properties.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

